ExpressPass: End-to-End Credit-based Congestion Control for Datacenters

As link speeds increase in datacenter networks, existing congestion control algorithms become less effective in providing fast convergence. TCP-based algorithms that probe for bandwidth take a long time to reach the fair-share and lead to long flow completion times. An ideal congestion control algorithms for datacenter must provide 1) zero data loss, 2) fast convergence, and 3) low buffer occupancy. However, these requirements present conflicting goals. For fast convergence,flows must ramp up quickly, but this risks packet losses and large queues. Thus, even the state-of-the-art algorithms, such as TIMELY and DCQCN, rely on link layer flow control (e.g.,Priority-based Flow Control) to achieve zero loss. This paper presents a new approach, called ExpressPass, an end-to-end credit-based congestion control algorithm for datacenters. ExpressPass is inspired by credit-based flow control, but extends it to work end-to-end. The switches control the amount of credit packets by rate limiting and ensure data packets flow in the reverse direction without any loss. ExpressPass leverages this to ramp up aggressively. ExpressPass converges up to 80 times faster than DCTCP at 10Gbps link, and the gap increases as link speeds become faster. Our simulation with realistic workload shows that ExpressPass significantly reduces the flow completion time especially for small and medium size flows compared to DCTCP, HULL, and DX.

==> 03_feedback_algorithm.tex <==
\section{Credit Feedback Control}\label{sec:feedback}

As explained in Section~\ref{sec:design}, \sys use feedback control on the credit packets to achieve fairness and high-utilization. One might wonder how is doing feedback control makes it better than doing it in data plane. The fundamental difference comes from the cost of packet loss and queuing between credit and data packets. Because we use very small queue for credits, and losing credits or filling up credit queue have very little impact on end to end performance. This allows us to use very aggressive feedback control enabling fast convergence and high utilization with small queue. Moreover, it simplifies the feedback control problem much simpler by eliminating requirements of reduce queuing or excessive loss. 

\begin{algorithm}[t]
\caption {Credit Feedback Control at Receiver.}%\kj{define meaning of each variable and provide example f }}
\label{alg:credit-feedback}
  \begin{itemize}
    \setlength\itemsep{0.01em}
    \item[] \textbf{(Initialization)} $cur\_rate = initial\_rate$
    \item[] Per update period (RTT by default)%When receiver sends credit packet for every granularity
    \item[] \quad \textbf{if} credit loss detected
    %\item[] \qquad $cur\_rate = f_{down} (cur\_rate, average\_data\_rate)$
    \item[] \qquad  $cur\_rate = average\_data\_rate$
    \item[] \quad \textbf{else}
    %\item[] \qquad $cur\_rate = f_{up}(cur\_rate, max\_rate)$
    \item[] \qquad $cur\_rate = (cur\_rate+max\_rate)/2$
    \item[] \quad \textbf{endIf} 
  \end{itemize}
\end{algorithm}

\noindent
\textbf{Feedback control loop:}
Algorithm~\ref{alg:credit-feedback} describes the pseudo code for feedback control we used for experiments throughout the paper. It reduces the amount of credit if it detects that credit is being lost in the network. Otherwise, it increase the credit rate. Detecting credit loss is straightforward. Each credit carries a sequence number, and data packet carries back the corresponding credit sequence number. If there is a gap between in sequence, we consider it as a loss. This is designed without the reordering in the network, and we leave this part for future work.

Next is amount of increase and decrease. We use very aggressive change for both increase and decrease to achieve fast convergence. During the increase, it converges to mid point between maximum credit rate and the current rate. This allows it to ramp up to over 90\% of bandwidth in just 4 RTTs. For decrease, we simply reduce it down to amount of credit delivered to the sender during prior RTT, which is equal to the amount of data received.

\noindent
\textbf{Convergence:}
Now, we turn our attention to how this algorithm converges. Here, we give an intuition why this converge to fairness, but leave formal analysis as future work.
Suppose there are two flows (A and B) with credit rate of $R_A$ and $R_B$ respectively. Assume ratio between them is $r = {{R_A} \over {R_B}} < 1$, meaning the convergence is not reached. During the decrease phase, with high probability $R_A$ and $R_B$ will be decreased by the same factor, not changing the ratio at all. Randomized jitter helps to achieve this under drop tail queue by removing some synchronized effect similar to drop in RED queue. However, during the increase phase, new ratio will be ${{(R_A + C) / 2} \over { (R_B + C) / 2}} = {{R_A + C} \over {R_B + C}}$ where C is $max\_rate$. This is strictly larger than ${R_A} \over {R_B}$ but smaller than 1. The algorithm then will eventually converge towards $r=1$. One assumption here is that $max\_rate$ is the same across all flows. This may not necessarily true, if datacenter uses different link speed for different host. It is possible to use the largest rate for flows in lower link speed. We leave the generalization and analysis as a future work.


%\begin{itemize}
%\item Our feedback control's objective is slightly different than data plane, as we don't care about loss / overflowing token queue as long as it converges to fairshare quickly.
%\item We need to explain why it congerge? algorithm we propose here.
%\item We also need to explain why it converge faster than others could do.
%\end{itemize}

%\noindent
%\textbf{Detecting credit loss:}
%\ds{need to rewrite}
%By receiver's sending credit packets at its fair-share rate, fairness and link utilization of C3 can be improved in multi-bottleneck topology and parking lot topology.
%To make receiver sends credit packets at its fair-share rate, we designed credit feedback control algorithm which use credit packet loss as congestion signal. Because every credit packet has its own credit sequence number and returning data packet echos received credit sequence number, receiver can know whether certain credit packet has been dropped or not by examining credit sequence number of received data packet.

\noindent
%\textbf{Transmitting credit packets:}
%when do you send? (3-way handshake)
%ACK-piggy backing. 





%\noindent
%\textbf{Algorithm:}
%Our rate feedback algorithm tries to estimate the fair-share, just like any other congestion control. One key difference is that, unlike traditional reactive algorithms, over-estimation in credit-based congestion control only results in utilization loss as oppose to latency increase commonly observed in traditional algorithms. In contrast, under-estimating the fair-share usually results in latency increase because it takes longer to ramp up to the fair-share. Thus, we make an intentional trade-off to become more aggressive in favor of reducing latency.  

%Algorithm~\ref{alg:credit-feedback} describes our algorithm. $cur\_rate$ is current credit sending rate, $average\_data\_rate$ is average data packet arrival rate for previous update period, and $max\_rate$ is the maximum credit sending rate corresponding to line rate at the receiver. For every update period (RTT), if credit packet loss have been detected, it reduce the credit sending rate with a function of current credit sending rate and average data arrival rate. On the other hand, if credit packet loss have not been detected, which means there may exist available bandwidth, it raises its credit sending rate with a function of current credit sending rate and maximum credit sending rate. For example, if credit has been lost one can update current rate into average data arrival rate ($cur\_rate = average\_data\_rate$) and if credit loss have not been detected one can update current rate into the average of current rate and maximum credit rate ($cur\_rate = (cur\_rate+max\_rate)/2$). \ds{rewrite}
 
 

\iffalse
On designing the function $f_{down} ()$ and $f_{up} ()$, enough care should be taken. With absence of the congestion signal if we raise the credit sending rate too aggressively (e.g. just set credit sending rate into maximum rate), it can result in unfairness and bandwidth waste. On the other hand, if we raise the credit sending rate too cautiously (e.g. sending one more credit per RTT) it will take much longer time to converge to the fair-share point. Similarly with the presence of congestion signal if we reduce the credit sending rate too aggressively, there will be under-utilization of the bandwidth or require much queue space to compensate it. On the other hand, if we reduce the credit sending rate too cautiously, credit feedback control algorithm will not do a much role in addressing fairness and bandwidth waste problem because it takes longer time to reach its fair-share rate.
\fi


